EUV and X-ray Spectroscopy of the Active Sun

This thesis strives to improve our understanding of solar activity, specifically the behaviour of solar flares and coronal mass ejections. An investigation into the hydrodynamic evolution of a confined solar flare was carried out using RHESSI, CDS, GOES and TRACE. Evidence for pre-flare heating, explosive and gentle chromospheric evaporation and loop draining were observed in the data. The observations were compared to a 0-D hydrodynamic model, EBTEL, to aid interpretation. This led to the conclusion that the flare was not heated purely by non-thermal beam heating as previously believed, but also required direct heating of the plasma. An observational investigation in to the initiation mechanism of a coronal mass ejection and eruptive flare was then carried out, again utilising observations from a wide range of spacecraft: MESSENGER/SAX, RHESSI, EUVI, Cor1 and Cor2. Observations provided evidence of CME triggering by internal tether-cutting and not by breakout reconnection. A comparison of the confined and eruptive flares suggests that while they have different characteristics, timescales and topologies, these two phenomena are the result of the same fundamental processes. Finally, an investigation into the sensitivity of EUV imaging telescopes was carried out. This study established a new technique for calculating the sensitivity of EUV imagers to plasmas of different temperatures for four different types of plasma: coronal hole, quiet sun, active region and solar flare. This was carried out for six instruments: Proba-2/SWAP, TRACE, SOHO/EIT, STEREO A/EUVI, STEREO B/EUVI and SDO/AIA. The importance of considering the multi-thermal nature of these instruments was then put into the context of investigating explosive solar activity.

==> 0_frontmatter/glossary.tex <==
% this file is called up by thesis.tex
% content in this file will be fed into the main document

% Glossary entries are defined with the command \nomenclature{1}{2}
% 1 = Entry name, e.g. abbreviation; 2 = Explanation
% You can place all explanations in this separate file or declare them in the middle of the text. Either way they will be collected in the glossary.

% required to print nomenclature name to page header
\markboth{\MakeUppercase{\nomname}}{\MakeUppercase{\nomname}}


% ----------------------- contents from here ------------------------

% chemicals
\nomenclature{\emph{SOHO}}{} 
\nomenclature{\emph{STEREO}}{}
\nomenclature{MDI}{}
\nomenclature{NASA}{}
\nomenclature{ESA}{}
\nomenclature{EUVI}{}
\nomenclature{LOS}{}
\nomenclature{LFF}{}
\nomenclature{NLFF}{Non-linear Force Free}





==> 6/swap stuff/ch6.tex <==
\chapter{Temperature response of EUV imagers}
\label{chapter:swap}
\section{Introduction}
\label{section:swap_intro}

Extreme ultraviolet imagers have revolutionised the way we look at the Sun. The highly dynamic nature of the solar corona was first conveyed by EIT on board SOHO (e.g. Moses et al. 1997). With a nominal cadence of ~10 minutes and a plate scale of 2.6Ó/pixel this instrument paved the way for the assortment of imagers in use today (Delaboudinire et al. 1996). Since then, the cadence and resolution of EUV imagers have improved. The TRACE instrument (Handy et al. 1999) has a small field-of-view (512Ó x 512Ó), but its 0.5Ó/pixel plate scale provides high resolution views of the solar corona. While the EUVI instruments on board the STEREO spacecraft do not have quite as high resolution as TRACE, their high cadence and full sun capability has broadened the scope of EUV imagers (Howard et al. 2008). The AIA instrument on board SDO, due to be launched in November 2009, will supply the community with 0.1 second cadence and 0.6Ó/pixel images (Smith et al. 2006). 

The optical set up of these instruments result in sensitivity to a wavelength range of typically 20 - 30 \AA. While the optical response is based around a dominant emission line at a well known temperature in that wavelength range, it is not surprising that neighbouring emission lines at widely varying temperatures can have a significant contribution, often contaminating images. It is very important to get a full and complete understanding of the behaviour of the instrument optics, both as a function of wavelength and of temperature. Often this is done theoretically (reference some other instrument, euvi maybe??). The quantum efficiency (the fraction of photons hitting a detector that are actually detected) combined with the transmission of the filters and reflection of the mirrors (!!!!!!!!!!!!!!!!! FIX THIS!!!!!!!!!!!!!!) give rise to the theoretical output signal of the instrument. It is also possible to achieve this by tuning a synchrotron beam across the wavelength range and measuring the throughput as a function of wavelength. 

This chapter is dedicated to the analysis of the SWAP instrument on board the ESA PROBA2 spacecraft that was launched in November 2009. SWAP is an EUV imager with a single filter centered on the 171 \AA \ \ion{fe}{ix} line. The instrument, which is laid out in Fig. \ref{fig:swap} has a 54$\arcsec$ field of view, larger than any other EUV spacecraft. It is one of a pair of instruments, the other being the solar irradiance monitor LYRA (hochedez et all 2009???????????). The temperature response of the SWAP instrument was calculated for four different circumstances - coronal hole, quiet sun, active region and solar flare. The discrepency between these is important as the solar spectrum for each is dramatically different, especially in the flaring scenario. These results were then compared to those of the other EUV instruments currently in operation - SOHO/EIT, TRACE, STEREO A/EUVI, STEREO B/EUVIB and SDO/AIA. 


\begin{figure}[!h]
\centering
\includegraphics[width=0.8\textwidth, trim = 0  0 0  0, clip = true]{swap_layout.pdf} 
\caption{The SWAP instrument layout with beam path highlighted in yellow. Top right shows a sample image from the BESSY synchrotron run. }
\label{fig:swap}
\end{figure}


This probably needs more.

\section{Wavelength calibration}
This study began with the analysis of BESSY synchrotron data. This required analysis and reduction of the ``beam'' data. Data reduction involved subtraction of dark frames and time normalisation as follows:

The beam strength ($I_{beam}$, [\emph{$phot \ s^{-1}$}]) before passing through the instrument optics was available from the instrument data. This is shown in the schematic in Fig. \ref{fig:swap}. Following transmission, the detected signal ($I_{det}$, Fig. \ref{fig:swap}) was calculated as the total number of detections (measured in data numbers - DN) per second over the entire detector:


\begin{equation}
\label{eqn:counts_cal}
I_{det} =  \frac{1}{exp\  time} \int \!\!\! Counts \ \,d pix    \hspace{3.8cm}   [DN\ s^{-1}]
\end{equation}

The instrument response was then given as the ratio of the detected signal to the input signal (i.e. what you must multiply the detected signal by to achieve the initial input).

\begin{equation}
\label{eqn:cal}
Instrument\ response =  \frac{I_{det}}{I_{beam}}  \hspace{2.2cm}   [DN\ phot^{-1}].
\end{equation} 

The instrument response was then adjusted for distance from the Sun and aperature size. The fraction of light observed by one pixel is given by the area of the aperature $[cm^{2}]$ times the steradian coverage of one pixel $[str\ pix^{-1}]$. 


\begin{figure}[!h]
\centering
\includegraphics[width=0.6\textwidth, trim = 0  0 0  0, clip = true]{steradian.pdf} 
\caption{Steradian coverage of one pixel based.}
\label{fig:ster}
\end{figure}

\begin{itemize}
\item Original spectrum:   $[DN phot^{-1}]$ 
\item Aperture area:  $\pi r^{2} = \pi \times 1.65^{2} \  [cm^2]$
\item Steradian coverage of one pixel: 	$\left([pix\ length''] \times [arcsec \to degrees] \times [degrees \to radians] \right)^{2} \\
 = \left( 3.1'' \times \frac{1}{60\times 60} \times \frac {\pi}{180}\right)^{2} \ [str \ pix^{-1}]$ 
\item New response units: $[DN \ phot^{-1} \ cm^{2} \ str \ pix^{-1} ]$. 
\end{itemize}


Multiplying the calibrated response curve by the theoretical spectrum (in units of $[phot \ cm^{-2} \ str^{-1} \ s^{-1} ]$ gives the transmitted spectrum in units of $[DN \ s^{-1} \ pix^{-1} ]$. 



\begin{figure}[!h]
\centering
\includegraphics[width=1\textwidth, trim =0 50 0 20, clip = true]{swap_resp_cal_uncal.pdf} 
\caption{Instrument response for wavelength (linear)}
\label{fig:resp_lin}
\end{figure}


The calibration curves, both ``raw'' and calibrated are shown on both linear and log plots in Figs. \ref{fig:resp_lin}. The calibrated plots are also interpolated to give a higher resolution for comparison to spectra.



\section{Theoretical Spectra}
The assessment of the instrument response to temperature required the solar spectrum at temperatures covering the expected range, in this case $10^{4}$ to $10^{8}$~MK. There are a number of ways to obtain the spectra, most of which involve the use of the spectral analysis package CHIANT \citep{Dere97, Landi06}. A popular method (e.g. REFERENCE PAPERS HERE) is to investigate the response for quiet sun, assuming no high temperature emission. This often gives a highly peaked function, centered on $\sim$1~MK for the ``171 \AA'' bandpass. It is also regularly assumed that the density of plasma remains constant as you change temperature. This, of course, is not true. It is well known that temperature and density are both dependent on height. Therefore, it must be assumed that as you look at higher and higher temperatures, you are looking at higher and higher altitudes, and therefore lower density. The density effects the value of emission measure, which the theoretical spectrum is sensitive to. 

The approach taken here is to use theoretical differential emission measure (DEM) curves to track the changing emission measure through temperature to calculate the theoretical spectrum for narrow temperature bands. 


The theoretical DEM curves, obtained from CHIANTI that were used in this study can be seen in the top panel of Fig. \ref{fig:DEM_cvs}. Since 

\begin{equation}
\label{eqn:dem}
EM =  \int n_{e}^2 dT
\end{equation}
then
\begin{equation}
\label{eqn:em}
EM =  \int \left(n_{e}^2 \frac{\partial h}{\partial T}\right) dT 
\end{equation}
so
\begin{equation}
\label{eqn:den}
EM =  \int_{T_{i}}^{T_{i+1}}  \left( DEM \right) dT \hspace{5cm}	[cm^{-5} ]. 
\end{equation}
Therefore, the emission measure can be obtained from the DEM curves at a given temperature by integrating over the temperature ste. The EM curves as a function of temperature can be seen in the bottom panel of Fig. \ref{fig:DEM_cvs}.

\begin{figure}[!h]
\centering
%from /Users/claire/Documents/phd/proba2/swap/spec/dem_em_plot_both.pro
\includegraphics[width=0.9\textwidth, trim =0 40 0 40, clip = true]{dem_em_cvs.pdf} 
\caption{Differential emission measure and Emission measure as a function of temperature for coronal hole, quiet sun, active region and flare.   }
\label{fig:DEM_cvs}
\end{figure}


The calculation of an isothermal spectrum requires, not only the temperature and emission measure at that temperature, but also a typical value of density for that spectrum. This has little effect on the resulting spectrum and serves merely as a guide for the initial density of the upper levels. The values used were:

The density assumed for each scenario are as follows:
\begin{itemize}
\item Coronal hole: $10^{5} cm^{-3}$ \citep{Guhat99}
\item Quiet sun: $10^{8.6} cm^{-3}$ \citep{Young05};
\item Active region: $10^{9.5} cm^{-3} $ \citep{Gallagher01};
\item Flare: $10^{11} cm^{-3}$ \citep{Raftery09}.
\end{itemize}

The SSWIDL routines \textsc{ch\_synthetic.pro} and \textsc{make\_chianti\_spec.pro} were used to make the isothermal synthetic spectra. Photoexcitation was included for all simulations. Free-free and free-bound continua were also included in all simulations. The ionization fractions were obtained from Mazzotta et al, and the abundances were taken to be coronal (i.e. 0.4 times the photospheric abundance). This is plainly justifiable for quiet sun, active region and flare scenarios. This can also be applied to coronal holes. Using Ne, which has the second highest first ionization potential, \citet{Doschek98} find that the Si/Ne abundance ratio in interplume polar coronal hole regions is about a factor of 2 greater than the photospheric value and is close to or the same as in coronal quiet sun regions. 

\begin{figure}[!h]
\centering
%from /Users/claire/Documents/phd/proba2/swap/spec/dem_em_plot_both.pro
\includegraphics[width=0.9\textwidth, trim =0 40 0 40, clip = true]{schematic.pdf} 
\caption{Top: Synthetic isothermal spectrum for quiet sun at 1~MK and 10$^{26}$~cm$^{-5}$ (black) and the SWAP wavelength response (red). Middle: Transmitted spectrum (convolution of the synthetic isothermal spectrum and instrument response). Bottom: The SWAP temperature response, calculated by integrating the transmitted spectrum over wavelength for a range of temperatures. }
\label{fig:schematic}
\end{figure}

The process of calculating the instrument response at a particular temperature T$_{i}$, begins by obtaiing the corresponding EM value from Fig. \ref{fig:DEM_cvs}. These values, along with the density (above) are used to calculate the theoretical isothermal spectrum (top panel of Fig. \ref{fig:schematic}, in this case at a temperature of 1~MK and an emission measure of 10$^{26}$~cm$^{-5}$). This spectrum is convolved with the SWAP wavelength response from Fig. \ref{fig:resp_lin} which gives the transmitted spectrum, shown in the middle panel of Fig. \ref{fig:schematic}. This is what the instrument is expected to see once the light from the sun passes through its optics. Integrating the transmitted spectrum over wavelength will give the total number of counts the instrument is expected to see in one second in one pixel at a particular temperature, shown in the bottom panel. This process is repeated, moving to the next temperature increment, T$_{i+1}$, until the entire temperature range has been covered. 



\begin{figure}[!h]
\centering
%from /Users/claire/Documents/phd/proba2/swap/spec/pot_more_trans_spec.pro
\includegraphics[width=\textwidth, trim =0 0 0 0, clip = true]{multi_trans.pdf} 
\caption{Sample transmitted spectra over the temperature range under investigation. The ion names of the strongest lines are listed also. }
\label{fig:trans}
\end{figure}




Figure \ref{fig:trans} shows a sample of transmitted isothermal spectra over the temperature range we are interested in. It is interesting to note the continuum contribution changing with temperature. The spectrum is dominated by continuum at lower ($\le10^{5}$~K) and higher ($> 10^{6.5}$~K) temperatures. 

This analysis was expanded to compare the response of other EUV imagers, including SOHO/EIT, TRACE, STEREOA/EUVI, STEREOB/EUVI and SDO/AIA. Each of the instruments' response as a function of wavelength were obtained, either from SSW routines or from the instrument teams. Not all responses were in the required units. Some instruments were calibrated, as shown in Table \ref{table:cal}, with the resulting, calibrated response functions shown in Fig. \ref{fig:all_resps}.  


\begin{center}
\begin{tabular}{|l|c|c|c|}
\hline
\multicolumn{4}{|c|}{Unit correction}\\ \hline
Instrument	&	Initial Units 	&	Correct for cm$^{2}$	&	 Correct for str pix$^{-1}$\\
			& 				& ($\pi \times r_{aperature}^{2}$) 			& (pix length''$ \times$ arcsec $\to$ radians) \\ \hline
TRACE		&	DN phot$^{-1}$ cm$^{2}$ str pix$^{-1}$	& -	&	-\\ \hline
EIT 			&	DN phot$^{-1}$ cm$^{2}$ str pix$^{-1}$	& -	&	-\\ \hline
EUVI			&	DN phot$^{-1}$& $\pi \times 0.98^{2}$ 		&	$ \left(\frac{1.4\pi}{180 \times 60^{2}}\right)^{2}$\\ 	\hline
AIA			&	DN phot$^{-1}$& $\pi \times 6^{2}$ 		&	$ \left(\frac{0.6\pi}{180 \times 60^{2}}\right)^{2}$\\ 	\hline
\end{tabular}
\label{table:cal}
\end{center} 	
	
	
	
	


\begin{figure}[!h]
\centering
%from /Users/claire/Documents/phd/proba2/swap/spec/compare_all_171.pro
\includegraphics[width=\textwidth, trim =0 80 100 150, clip = true]{wav_resp.pdf} 
\caption{Wavelength response of the individual instruments after being corrected for units.   }
\label{fig:all_resps}
\end{figure}




\begin{figure}[!h]
\centering
%from /Users/claire/Documents/phd/proba2/swap/spec/compare_all_171.pro
\includegraphics[width=\textwidth, trim =0 0 00 0, clip = true]{instr_resps.pdf} 
\caption{Instrument response to temperature for 6 EUV imagers in the 171 \AA \ passband. }
\label{fig:all_temps}
\end{figure}

The instrument response to temperature for SWAP, TRACE, EIT, EUVIA, EUVIB and AIA are shown in Fig. \ref{fig:all_temps}. Despite the significant differences in the various wavelength responses, the overall response of the instruments to temperature agree very well. Some slight differences occur and can can be explained as follows:
\begin{itemize}
\item \textbf{Stratification in temperature response}
	\begin{itemize}
		\item This is due to the different sensitivities to wavelength. Specifically, AIA has a significantly higher response. This is primarily due to its large aperture, allowing more photons to be captured. 
	\end{itemize}
\item \textbf{Increased AIA and TRACE sensitivity between 10$^{5.2}$ and 10$^{5.45}$~K.} 
	\begin{itemize}
		\item This is as a result of TRACE and AIA's peak sensitivity occurring at 172 \AA, the wavelength of strong \ion{O}{v} lines formed at approximately these temperatures (see Fig. \ref{fig:trans} where LogT = 5.2 for example). 
	\end{itemize}
	\item \textbf{Offset between AIA peak temperature and other instruments}
		\begin{itemize}
		\item The peak of the AIA temperature response occurs at 10$^{5.92}$~K, compared to an average of 10$^{5.98}$~K for other instruments. This shift to cooler temperatures occurs because firstly, the sensitivity of AIA at 171 \AA \ is almost 25\% less than at its peak (at 172 \AA). Therefore, the characteristic \ion{Fe}{ix} bandpass line that is formed at 1~MK is not as significant as the \ion{O}{iv} and \ion{O}{v} lines formed between 10$^{5.5}$ and 10$^{5.9}$~K around 172 \AA (see Fig. \ref{fig:trans} where LogT = 5.5 for example). 
		\end{itemize}
	\item \textbf{Decreased AIA sensitivity between 10$^{6.3}$ and 10$^{6.5}$.}
		\begin{itemize}
		\item This comes from reduced sensitivity to the cluster of \ion{Ni}{xv} lines formed around 10$^{6.4}$ between 175 and 180 \AA (see Fig. \ref{fig:trans} where LogT = 6.4 for example). All instruments except AIA have a flat response to wavelength in the range 175 to 180 \AA, while AIA has a quickly decreasing response, making it less sensitive to these lines. 
		\end{itemize}	
\end{itemize}


\section{Results}
The primary motivation behind this work was to assess the maximum exposure time for the SWAP instrument for various classes of solar activity. The result of this is shown in Fig. \ref{fig:counts}. Here the total expected counts for each instrument for coronal holes, quiet sun, active regions and flares are shown, along with the time to reach (SWAP) saturation. It is clear that SWAP can be expected to saturate for images of longer than one second for flares. However, provided no flares occur, it is unlikely SWAP will saturate for exposure times of less than 14 seconds. dot dot dot... see Raftery (phd thesis) for more ...


\begin{figure}[!h]
\centering
%from /Users/claire/Documents/phd/proba2/swap/spec/compare_all_171.pro
\includegraphics[width=\textwidth, trim =0 30 00 20, clip = true]{counts.pdf} 
\caption{The total counts per second for each instrument and the time it will take to reach 3500 counts.  }
\label{fig:counts}
\end{figure}




==> Latex/Classes/urlbst <==
#! /usr/bin/env perl
#
# Usage: ./urlbst.pl [--eprint] [--doi]
#    [--nohyperlinks] [--inlinelinks] [--hypertex] [--hyperref]
#    [input-file [output-file]]
# If either input-file or output-file is omitted, they are replaced by
# stdin or stdout respectively.
#
# See http://purl.org/nxg/dist/urlbst for documentation
#
# $Id: urlbst.in,v 1.8 2007/03/26 17:21:56 norman Exp $

$version = '0.6';
($progname = $0) =~ s/.*\///;
$mymarker = "% $progname";
$mymarkerend = "% ...$progname to here";
$myurl = 'http://purl.org/nxg/dist/urlbst';


$infile = '-';
$outfile = '-';

$addeprints = 0;     # if true (nonzero) we add support for eprints
$eprintprefix = 'arXiv:';	# make these settable with --eprint? syntax?
$eprinturl = 'http://arxiv.org/abs/';

$adddoiresolver = '0';
$doiprefix = 'doi:';
$doiurl = 'http://dx.doi.org/';

$makehref = 0;
$availablestring = "Available from: ";
$inlinelinks = 0;

$Usage = "$progname [--eprint] [--doi]\n    [--nohyperlinks] [--inlinelinks] [--hypertex] [--hyperref]\n    [--help] [input-file [output-file]]";

while ($#ARGV >= 0) {
    if ($ARGV[0] eq '--eprint') {
	$addeprints = 1;
    } elsif ($ARGV[0] eq '--doi') {
        $adddoiresolver = 1;
    } elsif ($ARGV[0] eq '--nohyperlinks') {
        $makehref = 0;
    } elsif ($ARGV[0] eq '--hypertex') {
	$makehref = 1;
    } elsif ($ARGV[0] eq '--hyperref') {
	$makehref = 2;
    } elsif ($ARGV[0] eq '--inlinelinks') {
        $inlinelinks = 1;
    } elsif ($ARGV[0] eq '--help') {
        print <<EOD;
urlbst version $version
    Usage: $Usage
      --eprint:       include support for `eprint' fields
      --doi:          include support for `doi' field
      --nohyperlinks  do not include active links anywhere
      --inlinelinks   add hyperlinks to entry titles
      --hypertex:     include HyperTeX-style hyperlink support
      --hyperref:     include {hyperref}-style hyperlink support
                      (generally better)
      --help:         print this help
    Input and output files may be given as `-' (default) to indicate stdin/out
EOD
        exit(0);
    } elsif ($ARGV[0] =~ /^-/) {
        die "Unrecognised option $ARGV[0]: Usage: $Usage\n";
    } elsif ($infile eq '-') {
	$infile = $ARGV[0];
    } elsif ($outfile eq '-') {
	$outfile = $ARGV[0];
    } else {
	die "Usage: $Usage\n";
    }
    shift(@ARGV);
}

if ($inlinelinks && $makehref == 0) {
    print <<'EOD';
Warning: --inlinelinks and --nohyperlinks were both specified (possibly
    implicitly).  That combination makes no sense, so I'll ignore
    --nohyperlinks and use --hyperref instead
EOD
    $makehref = 2;
}

$exitstatus = 0;		# success status

open (IN, "<$infile") || die "Can't open $infile to read";
open (OUT, ">$outfile") || die "Can't open $outfile to write";

# We have to make certain assumptions about the source files, in order
# to patch them at the correct places.  Specifically, we assume that
#
#   - there's a function init.state.consts
#
#   - ...and an output.nonnull which does the actual outputting, which
#         has the `usual' interface.
#
#   - we can replace
#           fin.entry
#       by
#           new.block
#           output.url    % the function which formats and displays any URL
#           fin.entry
#
#   - there is a function which handles the `article' entry type (this
#         will always be true)
#
#   - there is a function output.bibitem which is called at the
#         beginning of each entry type
#   - ...and one called fin.entry which is called at the end
#
# If the functions format.date, format.title or new.block are not defined (the
# former is not in apalike, for example, and the last is not in the
# AMS styles), then replacements are included in the output.
#
# All these assumptions are true of the standard files and, since most
# style files derive from them more or less directly, are true of most (?)
# other style files, too.
#
# There's some rather ugly Perl down here.  The parsing for
# brace-matching could probably do with being rewritten in places, to
# make it less ugly, and more robust.

print OUT "%%% Modification of BibTeX style file ", ($infile eq '-' ? '<stdin>' : $infile), "\n";
print OUT "%%% ... by $progname, version $version (marked with \"$mymarker\")\n%%% See <$myurl>\n";
print OUT "%%% Added webpage entry type, and url and lastchecked fields.\n";
print OUT "%%% Added eprint support.\n"   if ($addeprints);
print OUT "%%% Added DOI support.\n"      if ($adddoiresolver);
print OUT "%%% Added HyperTeX support.\n" if ($makehref == 1);
print OUT "%%% Added hyperref support.\n" if ($makehref == 2);
print OUT "%%% Original headers follow...\n\n";

$found{initconsts} = 0;
$found{outputnonnull} = 0;
$found{article} = 0;
$found{outputbibitem} = 0;
$found{finentry} = 0;
$found{formatdate} = 0;
$found{formattitle} = 0;
$found{newblock} = 0;

while (<IN>) {
    /^ *%/ && do {
        # Pass commented lines unchanged
        print OUT;
        next;
    };
    
    /^ *ENTRY/ && do {
	# Work through the list of entry types, finding what ones are there.
	# If we find a URL entry there already, object, since these edits
	# will mess things up.
	$line = $_;
	until ($line =~ /\{\s*(\w*)/) {
	    $line .= <IN>;
	}
	$bracematchtotal = 0;	# reset
	bracematcher($line);
	$line =~ /\{\s*(\w*)/;
	$found{'entry'.$1} = 1;
	print OUT $line;
	$line = <IN>;
	until (bracematcher($line) == 0) {
	    # XXX deal with multiple entries on one line
	    ($line =~ /^\s*(\w*)/) && ($found{'entry'.$1} = 1);
	    print OUT $line;
	    $line = <IN>;
	}
	if (defined($found{entryurl})) {
	    print STDERR "$progname: style file $infile already has URL entry!\n";
	    # print out the rest of the file, and give up
            print OUT $line;
	    while (<IN>) {
		print OUT;
	    }
	    $exitstatus = 1;
	    last;
	} else {
            print OUT "    eprint $mymarker\n    doi $mymarker\n    url $mymarker\n    lastchecked $mymarker\n";
	}
	print OUT $line;
	next;
    };

    /^ *FUNCTION *\{init\.state\.consts\}/ && do {
        # In the init.state.consts function, add an extra set of
        # constants at the beginning.  Also use this as the marker for
        # the place to add the init strings function.
        print OUT <<EOD;
STRINGS { urlintro eprinturl eprintprefix doiprefix doiurl openinlinelink closeinlinelink } $mymarker...
INTEGERS { hrefform inlinelinks makeinlinelink addeprints adddoiresolver }
% Following constants may be adjusted by hand, if desired
FUNCTION {init.urlbst.variables}
{
  "$availablestring" 'urlintro := % prefix before URL
  "$eprinturl" 'eprinturl := % prefix to make URL from eprint ref
  "$eprintprefix" 'eprintprefix := % text prefix printed before eprint ref
  "$doiurl" 'doiurl := % prefix to make URL from DOI
  "$doiprefix" 'doiprefix :=      % text prefix printed before DOI ref
  #$addeprints 'addeprints :=         % 0=no eprints; 1=include eprints
  #$adddoiresolver 'adddoiresolver :=     % 0=no DOI resolver; 1=include it
  #$makehref 'hrefform :=           % 0=no crossrefs; 1=hypertex xrefs; 2=hyperref refs
  #$inlinelinks 'inlinelinks :=        % 0=URLs explicit; 1=URLs attached to titles
  % the following are internal state variables, not config constants
  #0 'makeinlinelink :=     % state variable managed by setup.inlinelink
  "" 'openinlinelink :=     % ditto
  "" 'closeinlinelink :=    % ditto
}
INTEGERS { 
  bracket.state
  outside.brackets
  open.brackets
  within.brackets
  close.brackets
}
$mymarkerend
EOD
	$line = $_;
	until ($line =~ /\{.*\}.*\{/s) {
	    $line .= <IN>;
	}
	$line =~ s/(\{.*?\}.*?\{)/$1 #0 'outside.brackets := $mymarker
  #1 'open.brackets :=
  #2 'within.brackets :=
  #3 'close.brackets :=

 /s;
	print OUT $line;
	$found{initconsts} = 1;
	next;
    };

    /^ *EXECUTE *\{init\.state\.consts\}/ && do {
        print OUT "EXECUTE {init.urlbst.variables}\n";
        print OUT;
        next;
    };

    /^ *FUNCTION *\{new.block\}/ && do {
        $found{newblock} = 1;
    };

    /^ *FUNCTION *{output\.nonnull}/ && do {
	print OUT "$mymarker\n";
	print OUT "FUNCTION {output.nonnull.original}\n";
        copy_block();
	print_output_functions();
	$found{outputnonnull} = 1;
	next;
    };

    /FUNCTION *\{fin.entry\}/ && do {
        # Rename fin.entry to fin.entry.original (wrapped below)
        s/fin.entry/fin.entry.original/;
        $found{finentry} = 1;
        print OUT;
        next;
    };

    /^ *FUNCTION *{format\.date}/ && do {
	$found{formatdate} = 1;
	print OUT;
	next;
    };

    /^ *FUNCTION *{format\.title}/ && do {
        # record that we found this
	$found{formattitle} = 1;
        print OUT;
	next;
    };

    /^ *format\.b?title/ && do {
        # interpolate a call to setup.inlinelink
        print OUT "  title empty\$ 'skip\$ 'setup\.inlinelink if\$ $mymarker\n";
        print OUT;
        next;
    };

    /^ *FUNCTION *\{article\}/ && do {

	print_missing_functions();
	print_webpage_def();

	print OUT;
	$found{article} = 1;
	next;
    };

    /FUNCTION *\{output.bibitem\}/ && do {
        # Rename output.bibitem to output.bibitem.original (wrapped below)
        s/{output.bibitem\}/\{output.bibitem.original\}/;
 	$found{outputbibitem} = 1;
        print OUT;
        next;
    };

    print OUT;
};

if ($exitstatus == 0) {
    # Skip this if we've already reported an error -- it'll only be confusing
    foreach $k (keys %found) {
        if ($found{$k} == 0) {
            print STDERR "$progname: $infile: failed to find feature $k\n";
        }
    }
}

close (IN);
close (OUT);

exit $exitstatus;;






sub print_output_functions {
    print OUT "$mymarker...\n";

    print OUT <<'EOD';
% The following three functions are for handling inlinelink.  They wrap
% a block of text which is potentially output with write$ by multiple
% other functions, so we don't know the content a priori.
% They communicate between each other using the variables makeinlinelink
% (which is true if a link should be made), and closeinlinelink (which holds
% the string which should close any current link.  They can be called
% at any time, but start.inlinelink will be a no-op unless something has
% previously set makeinlinelink true, and the two ...end.inlinelink functions
% will only do their stuff if start.inlinelink has previously set
% closeinlinelink to be non-empty.
FUNCTION {setup.inlinelink}
{ makeinlinelink
    { hrefform #1 = % hypertex
        { "\special {html:<a href=" quote$ * url * quote$ * "> }{" * 'openinlinelink :=
          "\special {html:</a>}" 'closeinlinelink :=
          }
        { hrefform #2 = % hyperref
            { "\href{" url * "}{" * 'openinlinelink :=
              "}" 'closeinlinelink :=
              }
            'skip$
          if$ % hrefform #2 =
        }
      if$ % hrefform #1 =
      #0 'makeinlinelink :=
    }
    'skip$
 if$ % makeinlinelink
}
FUNCTION {add.inlinelink}
{ openinlinelink empty$
    'skip$
    { openinlinelink swap$ * closeinlinelink *
      "" 'openinlinelink :=
      }
  if$
}
EOD

    # new.block is defined elsewhere

    print OUT <<'EOD';
FUNCTION {output.nonnull}
{ % Save the thing we've been asked to output
  's :=
  % If the bracket-state is close.brackets, then add a close-bracket to
  % what is currently at the top of the stack, and set bracket.state
  % to outside.brackets
  bracket.state close.brackets =
    { "]" *
      outside.brackets 'bracket.state :=
    }
    'skip$
  if$
  bracket.state outside.brackets =
    { % We're outside all brackets -- this is the normal situation.
      % Write out what's currently at the top of the stack, using the
      % original output.nonnull function.
      s
      add.inlinelink
      output.nonnull.original % invoke the original output.nonnull
    }
    { % Still in brackets.  Add open-bracket or (continuation) comma, add the
      % new text (in s) to the top of the stack, and move to the close-brackets
      % state, ready for next time (unless inbrackets resets it).  If we come
      % into this branch, then output.state is carefully undisturbed.
      bracket.state open.brackets =
        { " [" * }
        { ", " * } % bracket.state will be within.brackets
      if$ 
      s * 
      close.brackets 'bracket.state :=
    }
  if$
}

% Call this function just before adding something which should be presented in 
% brackets.  bracket.state is handled specially within output.nonnull.
FUNCTION {inbrackets}
{ bracket.state close.brackets =
    { within.brackets 'bracket.state := } % reset the state: not open nor closed
    { open.brackets 'bracket.state := }
  if$
}

FUNCTION {format.lastchecked}
{ lastchecked empty$
    { "" }
    { inbrackets "cited " lastchecked * }
  if$
}
EOD
    print OUT "$mymarkerend\n";
}

sub print_webpage_def {
    print OUT "$mymarker...\n";

    # Some of the functions below call new.block, so we need a dummy
    # version, in the case where the style being edited doesn't supply
    # that function.
    if (! $found{newblock}) {
        print OUT "FUNCTION {new.block} % dummy new.block function\n{\n  % empty\n}\n\n";
        $found{newblock} = 1;
    }

    print OUT <<'EOD';
% Functions for making hypertext links.
% In all cases, the stack has (link-text href-url)
%
% make 'null' specials
FUNCTION {make.href.null}
{
  pop$
}
% make hypertex specials
FUNCTION {make.href.hypertex}
{ 
  "\special {html:<a href=" quote$ *
  swap$ * quote$ * "> }" * swap$ *
  "\special {html:</a>}" *
}
% make hyperref specials
FUNCTION {make.href.hyperref}
{ 
  "\href {" swap$ * "} {\path{" * swap$ * "}}" *
}
FUNCTION {make.href}
{ hrefform #2 =
    'make.href.hyperref      % hrefform = 2
    { hrefform #1 =
        'make.href.hypertex  % hrefform = 1
        'make.href.null      % hrefform = 0 (or anything else)
      if$
    }
  if$
}

% If inlinelinks is true, then format.url should be a no-op, since it's
% (a) redundant, and (b) could end up as a link-within-a-link.
FUNCTION {format.url}
{ inlinelinks #1 = url empty$ or
   { "" }
   { hrefform #1 =
       { % special case -- add HyperTeX specials
         urlintro "\url{" url * "}" * url make.href.hypertex * }
       { urlintro "\url{" * url * "}" * }
     if$
   }
  if$
}

FUNCTION {format.eprint}
{ eprint empty$
    { "" }
    { eprintprefix eprint * eprinturl eprint * make.href }
  if$
}

FUNCTION {format.doi}
{ doi empty$
    { "" }
    { doiprefix doi * doiurl doi * make.href }
  if$
}

% Output a URL.  We can't use the more normal idiom (something like
% `format.url output'), because the `inbrackets' within
% format.lastchecked applies to everything between calls to `output',
% so that `format.url format.lastchecked * output' ends up with both
% the URL and the lastchecked in brackets.
FUNCTION {output.url}
{ url empty$
    'skip$ 
    { new.block 
      format.url output
      format.lastchecked output 
    }
  if$
}

FUNCTION {output.web.refs}
{
  new.block
  output.url
  addeprints eprint empty$ not and
    { format.eprint output.nonnull }
    'skip$
  if$
  adddoiresolver doi empty$ not and
    { format.doi output.nonnull }
    'skip$
  if$
}

% Wrapper for output.bibitem.original.
% If the URL field is not empty, set makeinlinelink to be true,
% so that an inline link will be started at the next opportunity
FUNCTION {output.bibitem}
{ outside.brackets 'bracket.state :=
  output.bibitem.original
  inlinelinks url empty$ not and
    { #1 'makeinlinelink := }
    { #0 'makeinlinelink := }
  if$
}

% Wrapper for fin.entry.original
FUNCTION {fin.entry}
{ output.web.refs  % urlbst
  makeinlinelink       % ooops, it appears we didn't have a title for inlinelink
    { setup.inlinelink % add some artificial link text here, as a fallback
      "[link]" output.nonnull }
    'skip$
  if$
  bracket.state close.brackets = % urlbst
    { "]" * }
    'skip$
  if$
  fin.entry.original
}

% Webpage entry type.
% Title and url fields required;
% author, note, year, month, and lastchecked fields optional
% See references 
%   ISO 690-2 http://www.nlc-bnc.ca/iso/tc46sc9/standard/690-2e.htm
%   http://www.classroom.net/classroom/CitingNetResources.html
%   http://neal.ctstateu.edu/history/cite.html
%   http://www.cas.usf.edu/english/walker/mla.html
% for citation formats for web pages.
FUNCTION {webpage}
{ output.bibitem
  author empty$
    { editor empty$
        'skip$  % author and editor both optional
        { format.editors output.nonnull }
      if$
    }
    { editor empty$
        { format.authors output.nonnull }
        { "can't use both author and editor fields in " cite$ * warning$ }
      if$
    }
  if$
  new.block
  title empty$ 'skip$ 'setup.inlinelink if$
  format.title "title" output.check
  inbrackets "online" output
  new.block
  year empty$
    'skip$
    { format.date "year" output.check }
  if$
  % We don't need to output the URL details ('lastchecked' and 'url'),
  % because fin.entry does that for us, using output.web.refs.  The only
  % reason we would want to put them here is if we were to decide that
  % they should go in front of the rather miscellaneous information in 'note'.
  new.block
  note output
  fin.entry
}
EOD

    print OUT "$mymarkerend\n\n\n";
}


sub print_missing_functions {
    # We've got to the bit of the file which handles the entry
    # types, so write out the webpage entry handler.  This uses
    # the format.date function, which which many but not all
    # bst files have (for example, apalike doesn't).  So
    # check that we either have found this function already, or
    # add it.
    if (! $found{formatdate}) {
	if ($found{entrymonth}) {
	    print OUT <<'EOD';
FUNCTION {format.date}
{ year empty$
    { month empty$
	{ "" }
	{ "there's a month but no year in " cite$ * warning$
	  month
	}
      if$
    }
    { month empty$
	'year
	{ month " " * year * }
      if$
    }
  if$
}
EOD
	} else {
	    print OUT <<'EOD';
FUNCTION {format.date}
{ year empty$
    'skip$
    { %write$
      "(" year * ")" *
    }
  if$
}
EOD
  	}
	$found{formatdate} = 1;
    }

    # If the style file didn't supply a format.title function, then supply
    # one here (the {webpage} function requires it).
    if (! $found{formattitle}) {
	print OUT <<'EOD';
FUNCTION {format.title}
{ title empty$
    { "" }
    { title "t" change.case$ }
  if$
}
EOD
    $found{formattitle} = 1;
    }
}

# Utility function: Keep track of open and close braces in the string argument.
# Keep state in $bracematchtotal, return the current value.
sub bracematcher {
    my $s = shift;
    $s =~ s/[^\{\}]//g;
    #print "s=$s\n";
    foreach my $c (split (//, $s)) {
	$bracematchtotal += ($c eq '{' ? 1 : -1);
    }
    return $bracematchtotal;
}

# Utility function: use bracematcher to copy the complete block which starts
# on or after the current line.
sub copy_block {
    $bracematchtotal = 0;
    # copy any leading lines which don't have braces (presumably comments)
    while (defined ($line = <IN>) && ($line !~ /{/)) {
        print OUT $line;
    }
    while (defined ($line) && bracematcher($line) > 0) {
        print OUT $line;
        $line = <IN>;
    }
    print OUT "$line\n";	# print out terminating \} (assumed
    				# alone on the line)
}

